Towards Fluorescence-Guided Autonomous Robotic Partial Nephrectomy on Novel Tissue-Mimicking Hydrogel Phantoms

Autonomous robotic systems hold potential for improving renal tumor resection accuracy and patient outcomes. We present a fluorescence-guided robotic system capable of planning and executing incision paths around exophytic renal tumors with a clinically relevant resection margin. Leveraging point cloud observations, the system handles irregular tumor shapes and distinguishes healthy from tumorous tissue based on near-infrared imaging, akin to indocyanine green staining in partial nephrectomy. Tissue-mimicking phantoms are crucial for the development of autonomous robotic surgical systems for interventions where acquiring ex-vivo animal tissue is infeasible, such as cancer of the kidney and renal pelvis. To this end, we propose novel hydrogel-based kidney phantoms with exophytic tumors that mimic the physical and visual behavior of tissue, and are compatible with electrosurgical instruments, a common limitation of silicone-based phantoms. In contrast to previous hydrogel phantoms, we mix the material with near-infrared dye to enable fluorescence-guided tumor segmentation. Autonomous real-world robotic experiments validate our system and phantoms, achieving an average margin accuracy of 1.44 mm in a completion time of 69 sec.

==> figs/SBR/sbr_plot_2.tex <==
\definecolor{OIblack}{RGB}{0, 0, 0}
\definecolor{OIgreen}{RGB}{0, 158, 115}
\definecolor{OIblue}{RGB}{0, 114, 178}
\definecolor{OIlightblue}{RGB}{86, 180, 233}
\definecolor{OIyellow}{RGB}{240, 228, 66}
\definecolor{OIorange}{RGB}{230, 159, 0}
\definecolor{OIred}{RGB}{213, 94, 0}
\definecolor{OIpink}{RGB}{204, 121, 167}

\colorlet{BESO}{OIgreen}
\colorlet{MPD}{OIblue}
\colorlet{DPT}{OIorange}
\colorlet{DPC}{OIpink}
\def\mybarwidth{0.3cm}
\begin{figurehere}
\centering
\begin{tikzpicture}
\begin{scope}[local bounding box=plot box]
\begin{axis}[
    %axis equal image,
    name=SBRMetrics,
    ybar,
    ymin=0.5,
    ymax=12,
    %xshift=-0.3cm,
    symbolic x coords={Day 1, Day 7},
    xtick=data,
    xlabel={},
    ylabel={SBR},
    ytick distance=3,
    ylabel style={
        at={(-0.4cm, 0.5)},
    trim axis left,
    trim axis right,
    },
    width=0.6\columnwidth,
    height=0.5\columnwidth,
    x tick label style={
        rotate=0,
        anchor=north,
        inner sep=0pt,
        align=center,
        font=\footnotesize,
        text width=1cm,
    },
    y tick label style={
        font=\footnotesize,
    },
    xtick pos=bottom,
    bar width=\mybarwidth,
    ymajorgrids=true,
    yminorgrids=true,
    minor y tick num=1,
    major grid style={thick, black!30!white, dashed},
    minor grid style={ultra thin, black!20!white, dashed},
    major x tick style = transparent,
    minor y tick style = transparent,
    enlarge x limits=0.5,
    legend style={
        %overlay,
        at={(1.05,0.5)},
        anchor=west,
        legend columns=1,
        font=\small,
        /tikz/every even column/.append style={column sep=0.2cm},
        draw=white,
        },
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.15cm,0.2cm); },
    %legend entries={0.38\%, 0.97\%, 2.04\%},
    ]
    %\addlegendimage{empty legend}
    %\addlegendentry{\textbf{Concentration:}}

    % 0.38
    \addplot+ [
        fill=MPD,
        draw=MPD!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={MPD!10!black},
    ] coordinates {
        (Day 1, 6.1142) -= (0.0, 0.3158) += (0.0, 0.2001)
        (Day 7, 3.6548) -= (0.0, 0.2334) += (0.0, 0.1709)
    };
    \addlegendentry{0.38\%};

    % 0.97
    \addplot+ [
        fill=DPC,
        draw=DPC!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPC!10!black},
    ] coordinates {
        (Day 1, 8.3795) -= (0.0, 0.3340) += (0.0, 0.8034)
        (Day 7, 5.826) -= (0.0, 0.7479) += (0.0, 1.0464) 
    };
    \addlegendentry{0.97\%};
    
    % 2.04
    \addplot+ [
        fill=DPT,
        draw=DPT!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPT!10!black},
    ] coordinates {
        (Day 1, 11.1838) -= (0.0, 0.1946) += (0.0, 0.1472)
        (Day 7, 8.5695) -= (0.0, 0.5392) += (0.0, 0.3576)
    };
    \addlegendentry{2.04\%};
\end{axis}

\end{scope}


% First row of images
\node [anchor=north] (97 img) at ($(plot box.south) + (0.0cm, -0.3cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/97_3.png}};
\node [anchor=north east] (38 img) at ($(97 img.north west) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/38_1.png}};
\node [anchor=north west] (204 img) at ($(97 img.north east) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/204_1.png}};

% First row annotations
\node [anchor=south east, text=white, outer sep=0.1cm] at (38 img.south east) {0.38\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (97 img.south east) {0.97\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (204 img.south east) {2.04\%};

% Second row of images, shifted vertically below the first row
\node [anchor=north] (97 img2) at ($(97 img.south) + (0, -0.1cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/97_2_7.png}};
\node [anchor=north east] (38 img2) at ($(97 img2.north west) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/38_2_7.png}};
\node [anchor=north west] (204 img2) at ($(97 img2.north east) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/204_3_7.png}};

% Second row annotations
\node [anchor=south east, text=white, outer sep=0.1cm] at (38 img2.south east) {0.38\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (97 img2.south east) {0.97\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (204 img2.south east) {2.04\%};

\node [anchor=south, rotate=90] at (38 img.west) {Day 1};
\node [anchor=south, rotate=90] at (38 img2.west) {Day 7};

\end{tikzpicture}
\caption{
We create samples with different dye concentrations to evaluate the quality of the NIR signal. The correlation between dye concentration and \glsreset{sbr}\gls{sbr} is approximately linear. In cool and shielded storage conditions, the visibility of the dye degrades on average 29.70\% over seven days. 
}
\label{fig:sbr}
\end{figurehere}

==> figs/SBR/sbr_plot_old.tex <==

\definecolor{OIblack}{RGB}{0, 0, 0}
\definecolor{OIgreen}{RGB}{0, 158, 115}
\definecolor{OIblue}{RGB}{0, 114, 178}
\definecolor{OIlightblue}{RGB}{86, 180, 233}
\definecolor{OIyellow}{RGB}{240, 228, 66}
\definecolor{OIorange}{RGB}{230, 159, 0}
\definecolor{OIred}{RGB}{213, 94, 0}
\definecolor{OIpink}{RGB}{204, 121, 167}

\colorlet{BESO}{OIgreen}
\colorlet{MPD}{OIblue}
\colorlet{DPT}{OIorange}
\colorlet{DPC}{OIpink}
\def\mybarwidth{0.2cm}
\begin{figurehere}
\centering
\begin{tikzpicture}
\begin{scope}[local bounding box=plot box]
\begin{axis}[
    %axis equal image,
    name=SNRMetrics,
    ybar,
    ymin=0.5,
    ymax=22,
    xshift=-0.3cm,
    symbolic x coords={Day 1, Day 7},
    xtick=data,
    xlabel={},
    ylabel={SNR},
    ytick distance=5,
    ylabel style={
        at={(-0.6cm, 0.5)},
    trim axis left,
    trim axis right,
    },
    width=0.5\columnwidth,
    height=0.5\columnwidth,
    x tick label style={
        rotate=0,
        anchor=north,
        inner sep=0pt,
        align=center,
        font=\footnotesize,
        text width=1cm,
    },
    y tick label style={
        font=\footnotesize,
    },
    xtick pos=bottom,
    bar width=\mybarwidth,
    ymajorgrids=true,
    yminorgrids=true,
    minor y tick num=1,
    major grid style={thick, black!30!white, dashed},
    minor grid style={ultra thin, black!20!white, dashed},
    major x tick style = transparent,
    minor y tick style = transparent,
    enlarge x limits=0.5,
    legend style={
        %overlay,
        at={(1.2,1.05)},
        anchor=south,
        legend columns=4,
        font=\small,
        /tikz/every even column/.append style={column sep=0.2cm},
        draw=black,
        },
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.15cm,0.2cm); },
    %legend entries={0.38\%, 0.97\%, 2.04\%},
    ]
    \addlegendimage{empty legend}
    \addlegendentry{\textbf{Concentration:}}

    % 0.38
    \addplot+ [
        fill=MPD,
        draw=MPD!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={MPD!10!black},
    ] coordinates {
        (Day 1, 10.9696) -= (0.0, 0.5954) += (0.0, 0.9806)
        (Day 7, 6.8425) -= (0.0, 0.2457) += (0.0,0.5536)
    };
    \addlegendentry{0.38\%};

    % 0.97
    \addplot+ [
        fill=DPC,
        draw=DPC!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPC!10!black},
    ] coordinates {
        (Day 1, 15.5575) -= (0.0, 0.5797) += (0.0, 0.9025)
        (Day 7, 10.3693) -= (0.0, 1.5500) += (0.0, 1.5367)
    };
    \addlegendentry{0.97\%};
    
    % 2.04
    \addplot+ [
        fill=DPT,
        draw=DPT!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPT!10!black},
    ] coordinates {
        (Day 1, 19.7315) -= (0.0, 0.5882) += (0.0, 0.4305)
        (Day 7, 15.6858) -= (0.0, 0.4311) += (0.0, 0.4520)
    };
    \addlegendentry{2.04\%};
\end{axis}

\begin{axis}[
    name=SBRMetrics,
    at=(SNRMetrics.right of south east),
    anchor=left of south west,
    xshift=-3.8cm,
    ybar,
    ymin=0.5,
    ymax=12,
    symbolic x coords={Day 1, Day 7},
    xtick=data,
    xlabel={},
    ylabel={SBR},
    ylabel style={
        at={(-0.6cm, 0.5)},
    },
    width=0.5\columnwidth,
    height=0.5\columnwidth,
    x tick label style={
        rotate=0,
        anchor=north,
        inner sep=0pt,
        align=center,
        font=\footnotesize,
        text width=1cm,
    },
    y tick label style={
        font=\footnotesize,
    },
    xtick pos=bottom,
    ytick distance=2.5,
    bar width=\mybarwidth,
    ymajorgrids=true,
    yminorgrids=true,
    minor y tick num=1,
    major grid style={thick, black!30!white, dashed},
    minor grid style={ultra thin, black!20!white, dashed},
    major x tick style = transparent,
    minor y tick style = transparent,
    enlarge x limits=0.5,
    ]

    % 0.38
    \addplot+ [
        fill=MPD,
        draw=MPD!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={MPD!10!black},
    ] coordinates {
        (Day 1, 6.1142) -= (0.0, 0.3158) += (0.0, 0.2001)
        (Day 7, 3.6548) -= (0.0, 0.2334) += (0.0, 0.1709)
    };

    % 0.97
    \addplot+ [
        fill=DPC,
        draw=DPC!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPC!10!black},
    ] coordinates {
        (Day 1, 8.3795) -= (0.0, 0.3340) += (0.0, 0.8034)
        (Day 7, 5.826) -= (0.0, 0.7479) += (0.0, 1.0464) 
    };
    
    % 2.04
    \addplot+ [
        fill=DPT,
        draw=DPT!10!black,
        error bars/.cd,
        y dir=both,
        y explicit,
        error bar style={DPT!10!black},
    ] coordinates {
        (Day 1, 11.1838) -= (0.0, 0.1946) += (0.0, 0.1472)
        (Day 7, 8.5695) -= (0.0, 0.5392) += (0.0, 0.3576)
    };

\end{axis}
\end{scope}


% First row of images
\node [anchor=north] (97 img) at ($(plot box.south) + (0.5cm, -0.4cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/97_3.png}};
\node [anchor=north east] (38 img) at ($(97 img.north west) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/38_1.png}};
\node [anchor=north west] (204 img) at ($(97 img.north east) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/204_1.png}};

% First row annotations
\node [anchor=south east, text=white, outer sep=0.1cm] at (38 img.south east) {0.38\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (97 img.south east) {0.97\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (204 img.south east) {2.04\%};

% Second row of images, shifted vertically below the first row
\node [anchor=north] (97 img2) at ($(97 img.south) + (0, -0.1cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/97_2_7.png}};
\node [anchor=north east] (38 img2) at ($(97 img2.north west) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/38_2_7.png}};
\node [anchor=north west] (204 img2) at ($(97 img2.north east) + (0, 0.0cm)$) {\includegraphics[width=0.25\columnwidth]{figs/SBR/204_3_7.png}};

% Second row annotations
\node [anchor=south east, text=white, outer sep=0.1cm] at (38 img2.south east) {0.38\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (97 img2.south east) {0.97\%};
\node [anchor=south east, text=white, outer sep=0.1cm] at (204 img2.south east) {2.04\%};

\node [anchor=south, rotate=90] at (38 img.west) {Day 1};
\node [anchor=south, rotate=90] at (38 img2.west) {Day 7};

%\node[anchor=north] at ($(GLTMetrics.south) + (0, -0.8cm)$) {\small a) GLT};
\end{tikzpicture}
\caption{
Caption
}
\label{fig:sbr}
\end{figurehere}
